Honest Students from Untrusted Teachers: Learning an Interpretable Question-Answering Pipeline from a Pretrained Language Model

Explainable question answering systems should produce not only accurate answers but also rationales that justify their reasoning and allow humans to check their work. But what sorts of rationales are useful and how can we train systems to produce them? We propose a new style of rationale for open-book question answering, called \emph{markup-and-mask}, which combines aspects of extractive and free-text explanations. In the markup phase, the passage is augmented with free-text markup that enables each sentence to stand on its own outside the discourse context. In the masking phase, a sub-span of the marked-up passage is selected. To train a system to produce markup-and-mask rationales without annotations, we leverage in-context learning. Specifically, we generate silver annotated data by sending a series of prompts to a frozen pretrained language model, which acts as a teacher. We then fine-tune a smaller student model by training on the subset of rationales that led to correct answers. The student is "honest" in the sense that it is a pipeline: the rationale acts as a bottleneck between the passage and the answer, while the "untrusted" teacher operates under no such constraints. Thus, we offer a new way to build trustworthy pipeline systems from a combination of end-task annotations and frozen pretrained language models.

==> content/discussion.tex <==
\section{Discussion}
This paper shows how to train an \emph{honest student} to produce \emph{markup-and-mask rationales} for answers to open-book questions. The rationales are more expressive than traditional mask-based rationales because they include free-text decontextualizing markup that make it more likely for each sentence to stand on its own as an explanation. Furthermore, the rationales are faithful in the sense that the student model must first produce the rationale, and then discards all other information from the passage when answering the question. This results in rationales that are more likely to entail the predicted answer.

A key aspect of our approach is that we do not assume access to any example rationales. Rather, we produce candidate examples using in-context learning 
with the PaLM language model~\cite{chowdhery2022palm}, 
and then filter these examples based on whether they lead to a correct answer. We believe that this general strategy could support many types of multi-step reasoning, well beyond the markup-and-mask rationales that we consider here. This is important because while markup-and-mask rationales are more expressive than mask-only rationales, we found that on the QuoRef dataset there are many questions that still cannot be answered from any single-sentence rationale. In future work we will explore the capability of the teacher model to support even more expressive reasoning patterns, through richer prompt chains.

\paragraph{Limitations.} 
A number of limitations are highlighted by the error analysis in \autoref{sec:error-analysis}.
More generally, we have assumed that answers can be rationalized by a contiguous span of the passage, after applying query-independent markup. This is largely true for SQuAD, where the student models are nearly as accurate as the end-to-end model, which has access to the entire passage. But in the QuoRef examples, there remains a significant gap. This gap is partly explainable by multi-hop questions, for which no contiguous rationale can be provided, even with query-independent markup. It is therefore natural to ask whether the gap could be closed using more elaborate derivations, such as the application of query-\emph{specific} markup. Another limitation is that markup is provided in a single forward pass, making it impossible to handle cataphoric references --- for example, when an individual's name is revealed only at the end of a passage. From the perspective of evaluation, a limitation of this paper is that we do not explore alternative supervised solutions to generate decontextualizing markup, such as the application of existing coreference resolution systems. 

\paragraph{Future work.} There are a number of other directions for future work. Rather than simply filtering by the \fm of the resulting answer, we might treat all outputs of the language model as samples from a ``behavior policy'', which could then be used to learn a policy via offline reinforcement learning by computing importance weights~\cite{precup2000eligibility,levine2020offline}. Similarly, rather than considering only the one-best output from the large language model, it might be beneficial to consider the full beam of outputs, which would show alternative interpretations of the passage~\cite{wang2022rationale}. Another possibility for making better use of the training data would be for the teacher model to supplement the chain-of-thought prompting approach presented here with a post hoc "rationalization" step in which PaLM is asked only to justify the gold answer~\cite{jacovi-goldberg-2021-aligning,zelikman2022star}.

